CDStore: Toward Reliable, Secure, and Cost-Efficient Cloud Storage via Convergent Dispersal

We present CDStore, which disperses users' backup data across multiple clouds and provides a unified multi-cloud storage solution with reliability, security, and cost-efficiency guarantees. CDStore builds on an augmented secret sharing scheme called convergent dispersal, which supports deduplication by using deterministic content-derived hashes as inputs to secret sharing. We present the design of CDStore, and in particular, describe how it combines convergent dispersal with two-stage deduplication to achieve both bandwidth and storage savings and be robust against side-channel attacks. We evaluate the performance of our CDStore prototype using real-world workloads on LAN and commercial cloud testbeds. Our cost analysis also demonstrates that CDStore achieves a monetary cost saving of 70% over a baseline cloud storage solution using state-of-the-art secret sharing.

==> discussion.tex <==
\subsection{Discussion}
\label{subsec:summary}

We summarize how CDStore addresses our design goals in \S\ref{subsec:goal}. 

\paragraph{Reliability:}
CDStore can tolerate any $n-k$ out of $n$ cloud failures (either temporary or
permanent), for example, due to the CDStore server failure or the storage
backend failure.  This leverages the property of systematic Reed-Solomon codes
\cite{Reed60,Blomer95,Plank97,Plank05}, such that a CDStore client can always
reconstruct a CAONT package, and hence the original data, from $k$ available
clouds.  In addition, our CDStore implementation also tolerates CDStore client
failures by putting all file metadata on the server side (see
\S\ref{subsec:CDStore-client-metadata}).  
%If it fails, it can restore all its data from any $k$ out of $n$ clouds.  We
%discuss it in \S\ref{sec:implementation}. 
%Since all file data and metadata are maintained on the server side (see
%\S\ref{subsec:CDStore-client-metadata}), the CDStore client can restore all
%its files from any $k$ out of $n$ clouds. 

\paragraph{Security:} CDStore ensures confidentiality against outsider
attacks, provided that an attacker cannot gain unauthorized accesses 
to $k$ out of $n$ clouds.  It leverages AONT to ensure that no
information of the original secret can be inferred from less than $k$ shares.

CDStore also ensures confidentiality against insider attacks that
run the CDStore client software.  We discuss this from two perspectives.
First, consider the case where an attacker attempts to infer the data of other
users through deduplication occurrences. The attacker cannot succeed in such a
side-channel attack, since two-stage deduplication makes the deduplication
patterns independent across users' uploads.  Second, consider the case where
an attacker gains unauthorized accesses to a subset of clouds, such that it can
identify the deduplication status of the shares of different users and perform
brute-force dictionary attacks \cite{Bellare13b} inside the clouds.  However,
as long as the attacker compromises less than $k$ clouds, the mapping from the
secret (which requires $k$ shares to be decodable) to the compromised shares
(less than $k$ shares) is a many-to-one mapping, thereby complicating the
brute-force dictionary attacks. 

CDStore ensures integrity, since CAONT-RS encoding embeds a hash for each
secret.  The decoded secret can be verified against the embedded hash. 

\paragraph{Cost efficiency:} 
We argue that both intra-user and inter-user deduplications effectively
remove duplicates.  Intra-user deduplication eliminates duplicates of the same
user's data.  This is effective for backup workloads, since the same user
often makes repeated backups of the same data as different versions
\cite{Kaczmarczyk12}.  Inter-user deduplication further removes duplicates
of multiple users.  For example, multiple users within the same organization may
share a large proportion of business files.  Some workloads exhibit large
proportions of duplicates across different users' data, such as virtual disk
images \cite{Jin09}, workstation file system snapshots \cite{Meyer11}, and
backups \cite{Wallace12}.   The removal of duplicates translates to cost
savings, which we analyze in detail in \S\ref{subsec:cost-analysis}. 


